On The Empirical Effectiveness of Unrealistic Adversarial Hardening Against Realistic Adversarial Attacks

While the literature on security attacks and defense of Machine Learning (ML) systems mostly focuses on unrealistic adversarial examples, recent research has raised concern about the under-explored field of realistic adversarial attacks and their implications on the robustness of real-world systems. Our paper paves the way for a better understanding of adversarial robustness against realistic attacks and makes two major contributions. First, we conduct a study on three real-world use cases (text classification, botnet detection, malware detection)) and five datasets in order to evaluate whether unrealistic adversarial examples can be used to protect models against realistic examples. Our results reveal discrepancies across the use cases, where unrealistic examples can either be as effective as the realistic ones or may offer only limited improvement. Second, to explain these results, we analyze the latent representation of the adversarial examples generated with realistic and unrealistic attacks. We shed light on the patterns that discriminate which unrealistic examples can be used for effective hardening. We release our code, datasets and models to support future research in exploring how to reduce the gap between unrealistic and realistic adversarial attacks.

==> 5-text-old.tex <==

\section{\textbf{Text classification and adversarial fine-tuning}}
The first use case that we consider is natural language processing, in particular text classification. 
%Differently from images, two sentences can not be indistinguishable from each other to human readers. 
Morris et al. \cite{morris2020reevaluating} defines four type of constraints for a successful and realistic adversarial example in natural language tasks: \textit{ semantics, grammaticality, overlap, } and \textit{non-suspicion}.  Semantics ensures that the adversarial transformations do not change the meaning of the sentence. Grammaticality requires that the adversarial examples do not introduce any grammatical errors. For example, using a verb tense of the future for an event happening in the present. Overlap constraints restrict the similarity between original and generated text at the character level. Finally, non-suspicion constraints ensure that the adversarial text does not look suspicious. This constraint is mostly defined by context. For example, replacing a word in a modern English text with a synonym from the English of Shakespeare in an academic paper would raise suspicions. 
Problem space text attacks that do not respect \textit{grammaticality} constraints are not robust to preprocessing. They are easier to be discarded, considering that a simple grammar checker will revert the adversarial sentence to its original version. Hence, in this paper, we assume the sentences fed to the language models are previously filtered for their grammar. Therefore, the real and the stronger attack that we want to protect against are the attacks that respect all four constraints defined by Morris et al. \cite{morris2020reevaluating}. 

% However, a metric like edit distance can measure the level of perturbation applied to a sentence, similarly to $L_p$ norm for images. Edit distance $d(a, b)$ measures the minimum number of operations necessary to transform the string $a$ into $b$. However, edit distance does not ensure that the adversarial sample will look natural to the reader. 
% Attacks that do not respect grammar are easier to be discarded, considering that a simple grammar checker will revert the adversarial sentence to its original version. Hence, in this paper, we assume the sentences fed to the language models are previously filtered for their grammar. Therefore, the real and the stronger attack that we want to protect against are the attacks that respect all four constraints defined by  Morris et al. \cite{morris2020reevaluating} (Synonym Substitution attacks).

\subsection{EXPERIMENTAL PROTOCOL}

%\subsubsection{Attacks used for hardening}
\subsubsection{\textbf{Adversarial attacks}}\mbox{}

\textbf{Grammatically unconstrained attack: } We use the black-box attack named DeepWordBug attack by \cite{gao2018black} which is based on character substitution. DeepWordBug applies character substitution transformations to  the highest ranked words in order of influence to model decision. An example of a sentence transformed with DeepWordBug is given below: 

\noindent \textit{Original sentence:}%[a] 
 poorly executed comedy

\noindent \textit{DeepWordBug:}%[a] 
 pKorly executed comedy


\textbf{Grammatically constrained attack:} We use the black-box  TextFooler by \cite{jin2020bert}, and PWWS by \cite{ren2019generating} which are based on synonym replacements. Similarly to DeepWordBug, TextFooler ranks the words based on their importance and replaces top ranked words with semantically similar words. For the same sentence as in the example above, TextFooler for instance generates the adversarial sentence below:

\noindent \textit{TextFooler: }%[a]
faintly executed comedy 

Meanwhile, PWWS uses word saliency and prediction probability to decide the word to be substituted and the replacement order for the synonyms. Contrary to the attacks from character substitution category like DeepWordBug, synonum based attacks like TextFooler and PWWS  respect all four constraints defined by \cite{morris2020reevaluating}, hence they are more realistic. 

\subsubsection{\textbf{Datasets}}
For the evaluation we use three datasets: 1) Rotten Tomatoes movie reviews \cite{pang2005seeing}, 2) Offensive subset from TweetEval dataset \cite{barbieri2020tweeteval}, 3) AG News \cite{Zhang2015CharacterlevelCN}. For AG News, we use only 7.5k samples for hardening  and  1k samples for evaluation. Both Rotten Tomatoes and Tweet Offensive are binary sentiment analysis datasets, while AG News classifies news in four categories. A training sample in these datasets is an input that consists of one or more sentences. The datasets come with different characteristics of input lengths. The smallest dataset is Rotten Tomatoes with 18.49 words in average per input. The largest dataset is AG News with an average of 38.78 words per input. We give additional statistics of input lengths for the three datasets %related to mean, standard deviation, minimum and maximum 
in Table \ref{tab-text_dataset_char}.

\begin{table}[ht!]
\centering
\caption{Statistical values of input lengths for datasets}
\begin{tabular}{lllll} 
\toprule
Dataset               & Mean        & Std         & Min & Max  \\ 
\hline
Rotten Tomatoes~      & 18.49~ ~ ~~ & 8.58~ ~ ~~  & 1   & 51   \\
TweetEval (Offensive) & 22.12~ ~ ~~ & 15.21~ ~ ~~ & 2   & 104  \\
AG News               & 38.78~ ~ ~~ & 11.18~ ~ ~~ & 11  & 178  \\
\bottomrule
\end{tabular}
\label{tab-text_dataset_char}
\end{table}


\subsubsection{\textbf{Model}}
We are using DistilBERT \cite{sanh2019distilbert} base model (uncased) available in Hugging Face, because it achieves a comparable performance with BERT, but it is lighter and faster to train. This general pre-trained language model can be fine-tuned in any task. 

\subsubsection{\textbf{Hardening strategy}}

For hardening the models, we use one clean epoch at the beginning of the training process, followed up with four epochs where the training samples are the adversarial examples generated by either DeepWordBug or TextFooler. Hence, this is a case of adversarial fine-tuning with five epochs (1 clean epoch + 4 adversarial). 

To evaluate initial robustness in clean model, we perform normal training for 5 epochs. 


\subsubsection{\textbf{Evaluation}}

%To evaluate the results of hardening with DeepWordBug and TextFooler we use two  synonym substitution attacks  to. As a first attack, we use TextFooler and  as a second attack we have chosen PWWS. PWWS uses word saliency to decide the word to  be substituted and the replacement order. A second attack for the evaluation allows us to have an unbiased assessment when fine-tuning with TextFooler. 

For each fine-tuned model, we evaluate the clean and robust accuracy against DeepWordBug, TextFooler and PWWS. Similarly, for training, for all the attacks we use the default hyperparameters from TextAttack library.
For validation set, we use the default split provided by TextAttack with for Rotten Tomatoes (1066 samples) and TweetEval (Offensive) (1324 samples). For AG News, we select randomly 1000 samples. 

For RQ2, the budget hyper-parameter that we can control is the number of training epochs. We harden the model with DeepWordBug for up to 20 epochs, and record for each epoch the robust accuracy against adversarial examples generated by TextFooler and PWWS. 

In RQ3, we evaluate for the two binary datasets: Rotten Tomatoes and TweetEval (Offensive) the sentence embeddings from the last layer of the models. We have reduced data dimension to 30 with PCA and later generated 2-dimensional data with t-SNE.  

For a deeper analysis of the t-SNE clusters we evaluate two clustering metrics (Silhouette Score and Calinski-Harabasz Score) and compare the adversarial examples generated from DeepWordBug and TextFooler. \textit{Silhouette Score}  has a range of [-1, 1].  \textit{Calinski-Harabasz Score} has a range of [0, +$\infty$]. 

%We will focus our evaluation on not-normalized Calinski-Harabasz Score because  differences between different clusters are more visible. 


\subsection{RESULTS}
\subsubsection{\textbf{\textit{RQ1: What is the level of robustness provided by unconstrained hardening (DeepWordBug) compared to constrained/problem space hardening (TextFooler) ?}}}

\begin{table*}
\centering
\caption{Accuracy of clean and adversarially fine-tuned models expressed in \%. First column represents the accuracy on clean test set and the remaining columns represent the accuracy on adversarial examples generated based on the test set.}
\label{tab-text}
\begin{tabular}{llllll} 
\toprule
Dataset                                &                 & \multicolumn{3}{c}{Attacked by}      &                 \\ 
\hline
                                       & Trained against & -     & DeepWordBug & TextFooler     & PWWS            \\ 
\cline{2-6}
\multirow{3}{*}{Rotten tomatoes}       & Clean baseline  & 83.68 & 19.51       & 5.49           & 12.22           \\
                                       & DeepWordBug     & 83.4  & 28.68       & 9.34           & 19.57           \\
                                       & TextFooler      & 80.49 & 27.27       & \textbf{17.72} & \textbf{27.51}  \\ 
\cline{2-6}
\multirow{3}{*}{TweetEval (Offensive)} & Clean baseline  & 81.04 & 24.6        & 11.56          & 18.45           \\
                                       & DeepWordBug     & 77.11 & 55.44       & 19.2           & 28.01           \\
                                       & TextFooler      & 78.47 & 55.34       & \textbf{43.21} & \textbf{44.95}  \\ 
\cline{2-6}
\multirow{3}{*}{AG News}               & Clean baseline  & 89.6  & 19.53       & 16.07          & 32.37           \\
                                       & DeepWordBug     & 89.8  & 42.18       & 17.29          & 39.87           \\
                                       & TextFooler      & 89.9  & 28.36       & \textbf{26.14} & \textbf{45.72}  \\
\bottomrule
\end{tabular}
\end{table*}


Table \ref{tab-text} shows that %grammatically 
unconstrained fine-tuning using DeepWordBug robustifies all three models at similar scale. The accuracy on PWWS adversarial sentences increases +7.35\% (from 12.22\% to 19.57) for Rotten Tomatoes,  +9.56\% for TweetEval (Offensive) and +7.5\% for AG News. 

%The second method of fine-tuning, using adversarial samples from a grammatical constrained attack like TextFooler is more successful. The improvement against PWWS attack are +15.29\%, +26.5\%, and +13.35\% respectively.  
Fine-tuning with a constrained attack (TextFooler) improves the robustness against PWWS by 15.29\%, 26.5\%, and 13.35\% for Rotten Tomatoes, TweetEval and AG News respectively.
Fine-tuning with TextFooler outperforms fine-tuning with DeepWordBug by 7.94\%, 16.94\% and 5.85\% across the 3 datasets in terms of PWWS robust accuracy. 

Both have a negligible impact on the clean performance of the models (TextFooler fine-tuning has a slightly better clean accuracy for TweetEval and AG News than DeepWordBug fine-tuning). 


%The model trained on TweetEval (Offensive) is the model that benefits the most from replacing DeepWordBug with TextFooler in the fine-tunning process, with 16.94\% higher accuracy.
%\textbf{Grammatically constrained hardening is more effective than grammatically unconstrained hardening with an increased robust accuracy up to 16.94\%.}

\textbf{Grammatically constrained hardening is a more effective robustification than grammatically unconstrained hardening with an increased robust accuracy up to 16.94\% with negligeable impact on clean performance.}

% From the table, we see that TextFooler is a stronger attack than PWWS. The accuracies difference on PWWS and TextFooler adversarial examples is up to 16.3\% for the AG News dataset. Regarding the behaviour of the two attacks used for fine-tuning on clean models, we see that TextFooler is a stronger attack than DeepWordBug. This is more noticeable for Rotten Tomatoes and TweetEval (Offensive) dataset where the difference of the accuracies is 14.02\% and 13.04\% respectively.  For AG News the attacks perform similarly. The accuracy of the model in TextFooler adversarials is  only 3.46\% lower compared to DeepWordBug.

\subsubsection{\textbf{\textit{RQ2: Can a larger budget help increase the robustness of unconstrained hardening (DeepWordBug) to the same levels as constrained/problem space hardening (TextFooler)? }}}

We investigate if additional budget can bring the performance of fine-tuning with DeepWordBug at the same levels as fine-tuning with TextFooler. 
The results for the three datasets are shown in Figure \ref{fig-text-rq2}. 

The robust accuracy fluctuates for the first epochs and stabilizes after the 15th epoch. It remains however below the robustness achieved with TextFooler fine-tuning for 5 epochs. 
%The accuracy of the models in adversarial examples generated from both TextFooler and PWWS fluctuates for the first epochs and stabilizes after the 15th epoch. This effect is more visible in TweetEval (Offensive) dataset, where the highest jump in accuracy happens between the 3rd and 4th epoch (21.66\%).  At this point, the accuracy is only 5.88\% lower than the accuracy achieved by fine-tunning with TextFooler for 5 epochs. 

\textbf{Given up to 4x larger budget, grammatically unconstrained hardening (DeepWordBug) remains less effective than grammatically constrained hardening.}
 
\begin{figure*}[ht!]
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\linewidth]{figures/mr_rq2_pwws.png}
    \caption{Rotten Tomatoes}
  \end{subfigure}\hfill
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\linewidth]{figures/te_rq2_pwws.png}
    \caption{TweetEval (Offensive)}
  \end{subfigure}\hfill
    \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\linewidth]{figures/ag_rq2_pwws.png}
    \caption{AG News}
  \end{subfigure}
  \caption{Effect of fine-tuning  with DeepWordBug for an increasing number of epochs. Lines represent the accuracy of  adversarially fine-tuned models with DeepWordBug under TextFooler (red) and PWWS(green). Stars represent the accuracy of the model trained with TextFooler for 5 epochs under TextFooler (red) and PWWS(green).}
  \label{fig-text-rq2}
  \end{figure*}


\subsubsection{\textbf{\textit{RQ3: What are some properties of the generated adversarial examples that affect the hardening results ? }}}

We hypothesize that the adversarial examples generated with DeepWordBug and TextFooler show different patterns and that unconstrained examples of DeepWordBug do not cover the vulnerable space of the model as good as the constrained examples of TextFooler. 
%in their latent representation embedding and their distribution across the task classes.  

%To answer this RQ, we look into the adversarial examples generated from DeepWordBug and TextFooler on the test set of the two binary datasets: Rotten Tomatoes and TweetEval (Offensive).

% We exclude AG News, that has four classes and 
% its analyses is more complex. 

\paragraph{\textbf{Analysis of the embeddings of the adversarial examples}}

We investigate whether there is a relationship between the position of the sentence embeddings and the robust accuracy of the model. 
%For the test set, we visualize in Figure \ref{fig-text-rq3} the sentence embeddings from the last layer of the models. We have reduced data dimension to 30 with PCA and later generated 2-dimensional data with t-SNE. 
In Figure \ref{fig-text-rq3}, most of the adversarial examples for both DeepWordBug and TextFooler lay on the decision boundary between the two classes, which are marked on orange and blue for both datasets. However, the samples generated from DeepWordBug are closely grouped together, with  a dense concentration at specific areas. Meanwhile, TextFooler adversarial sentences have a wider spread throughout the decision boundary. 

This qualitative analysis suggests that hardening with TextFooler robustifies a larger portion of the space in comparison with hardening with DeepWordBug and therefore leads to higher robust accuracy.

% For example in subfigure b) we see that DeepWordbug sentence embedings are mostly located in two key areas: bottom-left and top-right. Meanwhile, the samples for TextFooler are have a larger spread in the top-right corner, without creating a polarity. For the TweetEval (Offensive) dataset we see in subfigure c) that TextFooler has majority of adversarial non-offensive sentences closer to the offensive class. DeepWordBug embeddings lay closer to the biggest concentration of non-offensive tweets. 
% Adversarial offensive tweets in subfigure d) seem to follow a similar pattern for both DeeepWordBug and TextFooler. The majority is  concentrated on top-middle part and the rest are spread through the decision boundary and offensive class.

\begin{figure*}[!ht]
  \begin{subfigure}{0.23\linewidth}
  \includegraphics[width=\linewidth]{figures/rotten_tomatoes_clean_both_embd_class_0.png}
    \caption{Rotten Tomatoes negative reviews}
  \end{subfigure}\hfill
  \begin{subfigure}{0.23\linewidth}
  \includegraphics[width=\linewidth]{figures/rotten_tomatoes_clean_both_embd_class_1.png}
    \caption{Rotten Tomatoes positive reviews}
  \end{subfigure}\hfill
    \begin{subfigure}{0.23\linewidth}
  \includegraphics[width=\linewidth]{figures/tweet_eval_clean_both_embd_class_0.png}
    \caption{TweetEval (Offensive) non-offensive tweets}
  \end{subfigure}\hfill
  \begin{subfigure}{0.23\linewidth}
  \includegraphics[width=\linewidth]{figures/tweet_eval_clean_both_embd_class_1.png}
    \caption{TweetEval (Offensive) offensive tweets}
  \end{subfigure}\hfill
  \caption{Sentence embeddings of initial inputs and adversarial }
  \label{fig-text-rq3}
  \end{figure*}


%The embeddings do not quantify the spread of adversarial examples, hence 
The qualitative analysis of the clusters in Table \label{tab-text-cluster}.

A greater gap in robust accuracy from clean models in Table \ref{tab-acc-class} does not necessarily result in better separated adversarial sentence embeddings between TextFooler and DeepWordBug in Table \label{tab-text-cluster}. The greatest robust accuracy gap between TextFooler and DeepWord bug happens for the  negative class in Rotten Tomatoes dataset. However, the best separated clusters of generated sentences between DeepWordBug and TextFooler in Table \ref{tab-text-cluster} is the non-offensive class in TweetEval (Offensive) dataset. 


 \textbf{DeepWordBug generates adversarial embeddings with a higher concentration in the embedding space compared to TextFooler. The class where adversarial embeddings of DeepWordBug are better clustered in relation to adversarial embeddings from TextFooler, is not the  class where the robust accuracy differs the most.} 

% Another observation is that the classes that have a lower clustering accuracy between initial clean samples and the adversarial ones  will have higher robust accuracy. 


\begin{table}[ht!]
\centering
\caption{Clustering scores for adversarial samples generated by DeepWordBug and TextFooler for each class. A higher score indicates better clustering for both metrics.}
\begin{tabular}{lllll} 
\toprule
Dataset                                    & Class         & Clusters      & Silhouette & CH \\ 
\hline
\multirow{6}{*}{RT } & Negative      & DWB - TF      & -0.01      & 7.64               \\
                                           &               & Initial - DWB & 0.09       & 42.55              \\
                                           &               & Initial  - TF & 0.08       & 62.61              \\
                                           & Positive      & DWB - TF      & 0.02       & 11.66              \\
                                           &               & Initial - DWB & 0.15       & 171.31             \\
                                           &               & Initial - TF  & 0.12       & 131.36             \\
                                           &               &               &            &                    \\
\multirow{6}{*}{\rotcell{Tweet}} & Non-offensive & DWB - TF      & 0          & 23.01              \\
                                           &               & Initial - DWB & 0.04       & 36.78              \\
                                           &               & Initial - TF  & 0.06       & 78.99              \\
                                           & Offensive     & DWB - TF      & 0          & 1.48               \\
                                           &               & Initial - DWB & 0.11       & 94.86              \\
                                           &               & Initial - TF  & 0.09       & 82.95              \\
\bottomrule
\end{tabular}
\label{tab-text-cluster}
\end{table}




\paragraph{\textbf{Robustness according to each class}}


\begin{table*}[ht!]
\centering
\caption{Accuracy of clean and adversarially fine-tuned models for each class (in \%)}
\begin{tabular}{llllll} 
\toprule
Dataset               & Trained against & Class         & DeepWordBug/Improv  & Textfooler/Improv        & $\Delta$ TextFooler, DeepWordBug  \\ 
\hline
Rottten Tomatoes & Clean           & Negative      & 38.88               & \textbf{8.54}            & -30.34                     \\
                      &                 & Positive      & \textbf{0.22}       & 2.46                     & 2.24                       \\
                      & Deepwordbug     & Negative      & 31.9 / -6.98        & \textbf{14.25 / }+5.71   & -17.65                     \\
                      &                 & Positive      & 25.5 / +25.28       & \textbf{4.47 /~}+2.01   & -21.03                     \\
                      & Textfooler      & Negative      & 43.1 / +4.22        & \textbf{23.57 / }+15.03  & -19.52                     \\
                      &                 & Positive      & 12.1 /~-11.88       & 12.1 / +~9.64            & 0                          \\
Tweet offensive       & Clean           & Non-offensive & 35.31               & \textbf{16.31}           & -19                        \\
                      &                 & Offensive     & \textbf{0.6}        & 0.91                     & 0.3                        \\
                      & Deepwordbug     & Non-offensive & 80.06 / +44.75      & \textbf{27.58 / +~}11.27 & -52.48                     \\
                      &                 & Offensive     & \textbf{0 /~}-0.06 & 0.32 /~-0.59          & 0.32                       \\
                      & Textfooler      & Non-offensive & 72.6 / +37.29       & \textbf{56.57 /~}+40.26   & -16.04                     \\
                      &                 & Offensive     & \textbf{0 /~}-0.6   & 0.4 /~-0.51              & 0.4                        \\
\bottomrule
\end{tabular}
\label{tab-acc-class}
\end{table*}

In RQ1 and RQ2 we were interested on the general improvement of robustness. However, from image domain we know that not all classes behave similarly during model hardening. Therefore, we study the robustness of the two classes separately. The results are given in Table \ref{tab-acc-class}


The first observation that we have from the table is that for RottenTomatoes the robust accuracy we saw in RQ1 comes almost evenly distributed for both classes. However, for TweetEval (Offensive), in clean model the offensive class is not robust at all (only 0.9\% accuracy). Fine-tunning the model does not help on increasing the robustness for this class, it is actually slightly worse (-0.59\% for DeepWordBug and -0.51\% for TextFooler). However, the non-offensive class benefits of a major improvement on robustness, especially when fine-tunned with TextFooler (+40.26\%).  One reason might be that the pool of offensive words is small and once the model learns to include them in non-offensive sentences during fine-tuning, it is able to later recognize the adversarial sentences as non-offensive.

\textbf{Classes are not equally robust to the attacks and profit differently from the hardening process.}

The results given in Table \ref{tab-acc-class} show the clean model for Rotten Tomatoes dataset is more robust on negative class for both DeepWordBug and TextFooler.  Similarly, for TweetEval (Offensive)  the model is more robust  in non-offensive class. For both datasets, fine-tunning with DeepWordBug  gives a better improvement in robust accuracy when evaluating with TextFooler for the  negative  (+5.71) and non-offensive class (+11.27).  Fine-tunning with TextFooler, provides a higher boost in accuracy for the same classes, respectively negative (+15.03) and non-offensive class (40.26\%). 
% As a reminder we are interested on the robustification against TextFooler as the more realistic attack.

\textbf{The results show that the classes that are already more robust, benefit most from the hardening process}

We investigate now how the robustness towards one or another attack affects the hardening process for each class. For Rotten Tomatoes the clean model is less robust to TextFooler than DeepWordBug in negative class. Fine-tuning with TextFooler improves the robust accuracy for this class by +15.03\% compared to only +5.71 \% by DeepWordBug. For TweetEval Offensive the clean  model is less robust to TextFooler as well. Similarly to the first dataset, fine-tunning with TextFooler gives a higher  improvement in robust accuracy (+40.26\%) compared to fine-tunning with DeepWordBug (+11.27\%). For the remaining two classes, positive  reviews  in Rotten Tomatoes and Offensive in TweetEval DeepWordBug the clean model is less robust against DeepWordBug. However, the difference is not significant, respectively only 2.24\% and 0.3\%. Fine-tuning with DeepWordBug in the first dataset does not give a higher improvement in robust accuracy compared to TextFooler (2.01\% vs 9.64\%). In the second dataset, there is a decrease in robust accuracy of -0.59\%, which is very similar to -0.51\% by TextFooler. 

\textbf{Classes that are less robust against TextFooler compared to DeepWordBug, benefit more when the model is fine-tuned with TextFooler rather than DeepWordBug}

Another observation is that the class, with the lower clustering score between the initial clean sentences and successful adversarial examples, is the most robust class. This holds true for both DeepWordBug and TextFooler in both datasets. For example for Rotten Tomatoes dataset the robust accuracy of the clean model on negative class against TextFooler is higher than positive class. In Table \ref{tab-text-cluster}, we see that the Calinski-Harabasz clustering score between initial sentences and generated adversarial sentences is lower for the negative reviews  (62.61) compared to positive reviews (131.36). Similar observation can be done for the other dataset and other classes. A lower clustering score means between the initial sentences and generated adversarial sentences means that the clusters are not well separated. The adversarial sentence embeddings are close to the initial ones and widely spread. 

\textbf{The class where the adversarial examples fall closer to the initial sentences are more robust, and the vice-versa.}


% For TweetEval (Offensive) dataset, the accuracy of the model is higher on  TextFooler generated non-offensive sentences. This again corresponds to a lower Calinski-Harabasz score of 78.99 compared to 82.95 for the other class. Similarly, the models have a  higher accuracy on negative and non-offensive class for DeepWordBug generated sentences. This corresponds to a lower Calinski-Harabasz score for the pair Initial-DWB for Rotten Tomatoes (42.55) and TweetEval (Offensive) 36.78. 




% In this section, we confirmed that not all the classes are similarly robust. Additionally, they react to fine-tunning differently. Some classes benefit from a great improvement in robust accuracy, and some of them do not get more robust even after fine-tunning. The analysis did not confirm our expectation that the less robust classes ( or the ones where DeepWordBug and TextFooler are more successful)  are the ones to benefit the most from fine-tunning. Actually, the results showed that the opposite was true. The classes that are more robust, get a higher robustness boost compared to a less robust class in a binary setting. Additionally, the results showed that the classes that are less robust to TextFooler compared to DeepWordBug are the classes that benefit more from fine-tunning with TextFooler rather than DeepWordBug. However, there was no evidence that the vice-versa holds.







\subsection{\textbf{Conclusions on Text Classification use case}}

For text classification, we used fine-tuning to harden three models build on three different datasets. The two attacks that we compared for fine-tuning were grammatically unconstrained DeepWordBug and grammatically constrained TextFooler. From the experiments we derived the main conclusions:

- Fine-tuning with grammatical constraints brings a better improvement in robustness compared to fine-tuning without grammatical constraints.\\
- There is no correlation between increasing the number of fine-tuning epochs for grammatically unconstrained attack and improvement of robustness.\\
- Not all the classes are equally  robust and profit equally from fine-tuning. Counter-intuitively,  the class where an attack is less successful, is the class that benefits the most from fine-tuning. \\
- A lower clustering score between the initial clean samples and successful samples means a higher robust accuracy.
 

==> 9-conclusion-old.tex <==

\section{Discussions and Conclusion}
% To be updated to remove "Discussions" section parts.
% Adversarial attacks are present in computer vision but as well in other domains like text, security, finance, cyber physical systems etc. Many of these domains have a set of constraints in problem space that are transferred to feature space as well. This gave the opportunity to design three types of attacks depending on the space where they operate: \textit{unconstrained feature space}, \textit{constrained feature space}, \textit{problem space}. This paper for the first time studies the effect that including the generated adversarial attacks by one of the methods mentioned above has in hardening of the models. We analysed three use cases: \textit{text classification}, \textit{botnet detection}, \textit{malware classification}. The characteristics of our studies for these three use cases can be found in Table \ref{tab-overview}. The results showed that the unconstrained hardening affects the robustness of the models at different levels. For malware classification, it did not improve the robustness against the problem space attacks, for text classification it improved the robustness in all three dataset we studied but still the improvement was not  at same level as the improvement that constrained hardening brought. Finally, the unconstrained training for botnet detection resulted successful,  increasing the robustness by 96\%. 


While adversarial training, retraining, and fine-tuning are common defenses for ML models in the computer vision domain, these methods are technically hard to apply in constrained domains due to the high computational cost required to generate realistic constrained adversarial examples.
In this paper, we compared for the first time the effectiveness of defense methods when using cheap unconstrained adversarial examples and when using expensive more realistic examples.
 We analysed three use cases: \textit{text classification}, \textit{botnet detection}, \textit{malware classification}. The characteristics of our studies for these three use cases can be found in Table \ref{tab-overview}. 
We showed that in the text use case, using attacks in the problem space that respect grammatical constraints is up to X\% more effective than attacks that do not respect these constraints. We obtain similar results in the malware domain where the problem space attack that directly manipulates byte code leads to a more robust model than the one manipulating the feature representation, no matter if the latter respect the constraints or not. 
On the contrary, in the botnet use case, examples generated in the unconstrained feature space are as effective as the ones generated in the constrained space to robustify the model.
It means that more expensive and more realistic adversarial examples are not always preferable to cheap and unconstrained examples when defending a model, as they increase the cost without further increasing the robustness.

We showed that even if we increase the budget of the less constrained attacks, the examples generated do not lead to a model as robust as the one augmented with constrained/problem space examples.

This shows that the budget allocated to the unconstrained attack is not the cause of the non-effectiveness of the defense.

To understand the difference of results across our different use cases, we studied some properties of adversarial examples generated in different spaces.
We found using the text use case that a lower clustering score between the initial clean samples and adversarial examples leads to higher robust accuracy when using defense methods. We showed that for malware, adversarial examples in the problem space are found across all the latent space, including close the clean examples, which is not the case of feature space adversarial examples. We also noticed that the unconstrained and constrained feature space attacks in the botnet perturb the features in a similar way and the examples land in the same region of the feature space. 
These results suggest that the effectiveness of adversarial examples for defense methods does not depend on the space used to generate them or whether they respect the constraints or not. It mostly depends on the distance between the generated example and the clean examples and whether the unconstrained attack perturbs similar features, with similar magnitude a constrained/problem space attack would.
A metric to compare two sets of adversarial examples generated with different techniques is the clustering score between the clean samples and the generated examples: a higher score leads to higher robust accuracy.

The generalization of the study is limited by the number of attacks available for each dataset. In a perfect scenario, we would be able to evaluate the 3 spaces (unconstrained, constrained, and problem space) for all datasets using multiple defense techniques (training, retraining, fine-tuning). However, the attacks are not available in the literature for every space and every dataset. Designing them would require domain knowledge and tremendous effort, if at all possible. Additionally, this would require a higher computational budget which we do not have. 

We saw that using expansive realistic examples in the defense does not necessarily improve the robustness of a model further than using non-realistic examples.
These results should be taken into consideration when attempting to robustify a model: using more expensive realistic examples may be a waste of resources, while using cheap unconstrained adversarial examples may give a false sense of robustness depending on the use case.
We hope that this paper will pave the way for future research studying the characteristics of adversarial examples generated in different spaces.





\begin{table*}
\centering
\caption{Characteristics overview of three use cases included in this study}
\begin{tabular}{lllll} 
\toprule
                  &                             & Text                      & Botnet               & Malware                  \\ 
\hline
Hardening         &                             & Adversarial fine-tuning   & Adversarial training & Adversarial re-training  \\
Model             &                             & Transformers (Distilbert) & FeedForward NN       & RandomForest             \\
Datasets          &                             & Rotten Tomatoes           & CTU-13               & PeWin                    \\
                  &                             & TweetEval (Offensive)     &                      &                          \\
                  &                             & AG News                   &                      &                          \\
Hardening attacks & Unconstrained feature space & DeepWordBug               & PGD                  & PGD/U-MoEvA              \\
                  & Constrained feature space   & \textbf{TextFooler }      & \textbf{FENCE }      & MoEvA                    \\
                  & Problem space               & N/A                       & N/A                  & \textbf{AIMED }          \\
\bottomrule
\end{tabular}
\label{tab-overview}
\end{table*}



==> related-old.tex <==
\section{Related work}
\label{sec:related}

\subsection{\texbf{Constrained adversarial attacks in feature space}}
Most of the constrained  attacks in feature space are an upgrade of traditional computer vision attacks like JSMA \cite{papernot2016limitations}, C\&W \cite{carlini2017towards} or FGSM \cite{goodfellow2014explaining}. The majority of these attacks are evaluated in Network Intrusion Detection Systems (NIDS) \cite{chernikova2019fence, sheatsley2020adversarial, teuffenbach2020subverting, tian2020exploring, sheatsley2021robustness}. Chernikova et al. \cite{chernikova2019fence} designed a general attack framework named  FENCE for constrained application domains. The framework includes an iterative gradient attack that updates features based on their family dependencies. FENCE is one of the frameworks that handles the largest type of constraints, resulting in realistic constrained feature space examples. However, despite being a general framework, adapting it to new domains requires rewriting most of its components according to the domain constraints. Similarly to \cite{chernikova2019fence}, Sheatsley et al.  \cite{sheatsley2020adversarial} use the concept of primary features to describe those features whose values define the range of some other features. They integrate constraint resolution into  JSMA  attack to limit feature values in the range dictated by their primary feature. Later on  for the same case study, Sheatsley et al. \cite{sheatsley2021robustness}, learned boolean constraints with Valiant algorithm and introduced Constrained Saliency Projection (CSP), an improved iterative version of their previous attack. For a predefined number of iterations, the attack selects the  most influential feature to perturb and projects it back to the constrained space. The bottleneck of this attack is the process of learning the constraints. Its runtime  scales exponentially with the
number of features. While studying attacks on NIDS, \cite{teuffenbach2020subverting} divided the features in groups based on the difficulty to attack them. They extend C\&W attack to consider weights in these groups and favour modifications on low weighted features, i.e. the independent features. This approach does not guarantee that the generated adversarial examples respect constraints. Instead, it hopes that only modifications in independent features will be enough to cause a wrong prediction. Tian et al. \cite{tian2020exploring} explores visually feature correlations between features pairs. If any correlation is observed, then the constraint equation is defined analytically  and a constraint matrix is generated dynamically according to the constraint set and the sign of the gradient. They update IFGSM so that the Hadambard product between the sign of the gradient and constraint matrix  restricts the size  and direction of perturbation to respect data correlations. Despite this  method being among the few that uses a large variety of constraints types, it can not handle relationships of more than two features. 

Other constrained attacks are applied to a variety of other domains. For example, the first constrained attack by \cite{kulynych2018evading} proposes a graphical framework where the nodes represent the feasible examples and the edges represent valid transformations for each feature. They evaluated their approach on Twitter bot detection and website fingerprinting. Despite the results, this A* based attack is practically infeasible in many large datasets due to its time complexity. \cite{li2020conaml} considers Cyber-Physical Systems, a domain that has inherited physical constraints. They take into account two use cases, water treatment attack detection and State Estimation in Power Grids. For both, they identify a series of linear constraints related to sensor measurements and craft a  best-effort search attack that would respect these constraints. This approach can not handle non-linear constraints. \cite{levy2020not} updates JSMA attack to take into account immutable features and feature distribution. They evaluated their approach in three different tasks: price of lodging (AirBnb), medical data ICU, credit risk. 
Their proposal handles very loose constraints like mutability and probability distributions. It does not consider inter-feature relationships,  hence there is no guarantee that the generated examples are valid. Ghamizi et al. \cite{ghamizi2020search} studies as well the robustness of credit-scoring models. They propose a genetic algorithm that encodes constraints as objectives to be optimized. They support a variety of linear, non-linear and statistical constraints as long as they can be expressed as a minimization problem. This approach requires giving a  weight to each objective in advance. The weights can be defined by a domain expert.  Meanwhile, \cite{cartella2021adversarial} proposes some modifications to three existing attacks: Zoo, Boundary attack, HopSkipJump. The modifications consider the following factors:  feature modifiability,  feature data types and feature importance. Similarly to \cite{levy2020not} they do not consider feature relationships, therefore the attacks can still generate unfeasible examples in feature space. 

You can find a complete list of constrained adversarial attacks and their properties in Table~\ref{tab-cons-attacks}. Despite that they all include constraints in adversarial generation process, many  handle only basic constraints like mutability or data type. This restricts the generated adversarial examples, but do not completely ensure that they are feasible and realistic.  Constrained attacks  that are easily adaptable to many application domains and at the same time support a large variety of constraints  are missing in the literature.


% The framework
% groups dependent features in families and updates them together
% and assigns a representative feature to each family. At every attack iteration, the  representative feature related to the feature of maximum gradient is selected. This feature is updated first, and the dependent features in the family are updated accordingly to respect the constraints.
\begin{table*}[ht!]
\centering
\caption{Adversarial attacks in feature space that consider domain constraints}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllll} 
\toprule
                                                  & Year & Use case                         & Threat model     & Method                                & Constraint type                 & Expansion to new domains    & Open source  \\ 
\midrule
\cite{kulynych2018evading}    & 2018 & Twitter bot                      & White \&  Black box & Graphical framework                   & Mutability                      & Define~                     & Yes          \\
                                                  &      & Website-fingerprinting           &                  &                                       & Range               & the transformation graph    &              \\ 
\hline
\cite{chernikova2019fence}       & 2019 & Botnet detection                 & White box        & Iterative Gradient Based               & Mutability, Range,              & Rewrite most~               & Yes          \\
                                                  &      & Malicious domain classification  &                  &                                       & Ratio,One-hot encoding          & of the components           &              \\
                                                  &      &                                  &                  &                                       & Statistical ,Linear, Non-linear &                             &              \\ 
\hline
\cite{ghamizi2020search}         & 2020 & Credit scoring                   & Grey-box         & Genetic Algorithm                     & Mutability, Range,              & Define constraints~         & Yes          \\
                                                  &      &                                  &                  &                                       & Ratio, One-hot-encoding,        & as a minimization problem   &              \\
                                                  &      &                                  &                  &                                       & statistical, linear, non-linear &                             &              \\ 
\hline
\cite{li2020conaml}              & 2020 & Water treatment attack detection & White \& Black box  & Best-Effort Search                    & Mutability,range                & Define constraints          & No           \\
                                                  &      & State Estimation in Power Grids  &                  &                                       & Linear, 
Simple non-linear      &                             &              \\ 
\hline
\cite{levy2020not}               & 2020 & Price of lodging (AirBnb)        & White-box        & Extended JSMA                         & Mutability, Range,              & Yes                         & No           \\
                                                  &      & Medical data ICU                 &                  &                                       &                                 &                             &              \\
                                                  &      & Credit risk                      &                  &                                       &                                 &                             &              \\ 
\hline
\cite{sheatsley2020adversarial}  & 2020 & NIDS                             & White-box        & Constrained Augmented JSMA            & Mutability,Range,               & Learn constraints~          & No           \\
                                                  &      &                                  &                  &                                       & Boolean                         & from data                   &              \\ 
\hline
\cite{teuffenbach2020subverting} & 2020 & NIDS                             & White-box        & Extended CW attack                    & Mutability                      & Define feature groups       & No           \\ 
\hline
\cite{tian2020exploring}         & 2020 & NIDS                             & White-box        & Constraint-based IFGSM                & Linear                          & Define constraints~         & No           \\
                                                  &      &                                  &                  &                                       & Addition boundary constraint,   & by visual exploration       &              \\
                                                  &      &                                  &                  &                                       & Zero multiplication constraint  &                             &              \\ 
\hline
\cite{cartella2021adversarial}   & 2021 & Fraud                            & Black box        & Modified Zoo, Boundary attack, HopSkipJump         & Mutability,Data type            & Define feature weights      & No           \\ 
\hline
\cite{sheatsley2021robustness}   & 2021 & NIDS                          & White-box        & Constrained Saliency Projection & Boolean constraints             & Learn constraints~          & No           \\
                                                  &      & Phishing                         &                  &                                       &                                 & through Valiant’s algorithm &              \\
\bottomrule
\end{tabular}}
\label{tab-cons-attacks}
\end{table*}


\subsection{\textbf{Problem space attacks}}
Problem space attacks design and application is complex. Generally it is easier to deal with digital objects than tangible ones, therefore there are more problem space attacks in digital world. \cite{anderson2018learning} used reinforcement learning to modify binary Windows PE files to evade  Windows malware detection engines. The adversarial agent plays in ten rounds a competitive game against the detector. The round starts with an initial malware sample that is modified by a set of functionality-preserving operations. If the detector is bypassed, then the round stops before the 10th iteration.  The generated adversarial files are not checked if they are valid, therefore many files can be corrupt. \cite{castro2019aimed} uses the same set of operations as \cite{anderson2018learning} combined with Genetic Algorithm and   to generate adversarial Windows PE files. The original malware is injected with a fixed number of perturbations to create the initial population for the genetic algorithm. In the contrary to \cite{anderson2018learning}, Castro et al. evaluates in each iteration if the modified samples are still functional in order to avoid corrupt files. Only valid files are then fed to the malware detector.  \cite{pierazzi2020intriguing}  introduce a new problem space attack for android malware detection. They initially collect a set of bytecodes (gadgets) from benign files through program slicing. At the attack stage, they select the most important features for the classifier and gadgets that include those features. The gadgets are then implanted on the malicious file.  By design, the generated files are functional. 
\cite{schonherr2020imperio} introduced Imperio, an attack that produce adversarial audio examples for speech recognition systems. The particularity of the Imperio is that the audio can be played in different room environments without the need to be tuned for that specific environment. Additionally, the attack does not require a direct line-of-sight between speaker and microphone. A problem space domain where there exists a large variety of adversarial attacks is text. There is a category of attacks like \cite{gao2018black, li2018textbugger, pruthi2019combating} that generate adversarial text by replacing/swapping characters in the most influential words. The drawback of this approach is that the generated sentences will not continue to be adversarial if they are sent to a grammar checker before going to a classifier as input. Other attacks instead of replacing characters, replace complete words with their synonymous \cite{jin2020bert, ren2019generating, li2020bert}. These attacks are less suspicious to human eyes, however if the number of replaced words is not controlled properly the sentence might lose its original meaning. 







% \cite{cheng2021packet} for the first time introduces an adversarial attack that creates network traffic on flow level but on packet level instead. They base their work on SeqGan and propose Attack-GAN. Attack-Gan is based in a Generator-Discriminator architechture. Inspired by NLP they see each byte as a token in a sentence. They use so word embedding to build the representation of network packets. The generator task is then to replace tokens such the a black-box NIDS classifies gets fooled. The results of NIDS are fed to the discriminator, which decides if the generated traffic is malicious adversarial traffic. They limit the mutability of some tokens in order to enforce the security domain constraints, hence functional packets.

% \cite{rosenberg2020query} generate adversarial malware against classifiers based on the sequence of API calls. To avoid injecting hard coded benign API calls in the file that can easily be detected, they use a generative adversarial network (GAN) to mimic benign sequences.


==> review_constrained.tex <==
\section{Constrained adversarial attacks: A systematic review}


\subsection{Method search, eligibility & selection}

To identify adversarial attacks that focus their work on constrained domains, we used the search terms "constrained adversarial attacks", "realistic adversarial attacks", "adversarial attack in tabular data" and limited the search to the year 2018.  Every search term showed respectively 17,200, 17,500, 16,100  results. We screened through the first 100 results of every search term, leaving us with 300 articles. We discarded from the title every results that was irrelevant. Then from the abstracts we discarded the samples that were related to attacks in problem space and not in constrained space. Then we discarded results that had only time constraints, resources constraints or other constraints not related to features. Finally, we discarded the studies that were generating constrained counterfactual examples. As a result of our selection process, we have 10 studies from 2018 that generate adversarial examples in constrained feature space. 


\subsection{White-box}
Most of the constrained white box attacks are an upgrade of traditional computer vision attacks like JSMA, C\&W or gradient based (FGSM and PGD). The majority of these attacks are evaluated in NIDS \cite{chernikova2019fence, sheatsley2020adversarial, teuffenbach2020subverting, tian2020exploring, sheatsley2021robustness}.

\textbf{FENCE}
\cite{chernikova2019fence}  designed a general attack framework named  FENCE for constrained application domains. FENCE requires as inputs a set of features families. A family is a number of features that have dependencies and need to be updated simultaneously. Each family has a pre-chosen representative feature. Once the feature families are defined, FENCE takes an iterative gradient approach to find adversarial samples that respect a range of mathematical constraints. In every iteration, the gradient of mutable futures is calculated and the feature with maximum gradient is picked. If this feature does not belong to any features' family, it is updated with the standard gradient update.  Otherwise, the function that updates features' families is called.  In this function the representative feature is updated first according to gradient values  and later the dependent features in the family are updated accordingly to respect the constraints.  If the resulting adversarial example falls outside the allowed perturbation size, the algorithm performs a binary search on the value of perturbation for the representative features and continues updating the dependent features accordingly until an adversarial that respects the distance is found. In case when an adversarial is found, the FENCE framework stops updating the samples before the number of iterations is exhausted. 


FENCE is a general approach and can support a wide range of feature relationships. It can support: a) dependencies that are domain specific like range, ratio and one-hot encoding, b) mathematical feature dependencies like statistical, linear, non-linear or a combination of them. Supporting all these type of feature relationships means that the generated examples are very restricted and realistic. Despite the methodology and the approach being general, adapting FENCE from one domain to another it is not straight-forward. Firstly, a domain expert knowledge is necessary for almost every step in designing the components of the approach. Their input is needed to determine the feature families, representative features, feature relationships and their update functions. Secondly, after these elements are defined, applying them to a new domain requires rewriting/coding most of the components of the framework. Currently, an open source version is provided which is a tailored implementation to botnet detection application. 



\textbf{Constrained-Saliency Projection} 
Sheatsley et al. in two different studies  \cite{sheatsley2020adversarial}, \cite{sheatsley2021robustness} proposes an extended version of Jacobian-based
Saliency Map Approach that is able to handle feature relationships \cite{papernot2016limitations}. JSMA is an iterative approach that at each step calculates saliency maps, which are indicators of how influential is a feature on misclassifying the input. A perturbation is applied to the most salient feature iteratively. In order to upgrade JSMA to a constrained version, first they added a little tweak to JSMA. Originally, JSMA requires the perturbation parameter to be either positive or negative. To relax this requirement and allow perturbations to both directions dynamically, they perturb a  feature if the target gradient and sum of non-target gradients are in opposing directions. This updated version of JSMA is named AJSMA where A stands for Adaptive. 

Sheatsley takes two different approaches in these two studies on discovering feature relationships and upgrading the AJSMA to handle constraints. 

Regarding constraints discovery, in the first study published in 2020 \cite{sheatsley2020adversarial} the constraints are inferred by a domain expert and expressed as first-order logic. They rely on the concept of primary and secondary features. Primary features are features whose values define the permissible range values for some other features. On the other hand, secondary features do not bring any limitation in value for other features. Primary features are
the predicates in logical expressions that determine the values that secondary features can have. The constraints take then the following form: 
"∀x ∈ X : x�� ⇒ (x1 ∈ Y1) ∧ (x2 ∈ Y2) ∧ · · · ∧ (x�� ∈ Y��)
"a constraint exists between a primary feature ��, and any other feature ��, if there exists at least one input in the training set where both �� and �� are seen together. ""


Meanwhile in the second study \cite{sheatsley2021robustness} they took an automated approach to discover constraints through data through Valiant’s Algorithm. Valiant's Algorithm starts with a set of possible constraints expressed as boolean clauses over the dataset X. For every inupt in the dataset, the constraints that are not satisfied by the input are discarded. At the the end we will receive a reduced set of constraints that are satisfied by all inputs. As Valiant's algorithm is intially desined for boolean features, Sheatsley et al. have proposed some modifications to handle categorical and real features. 

Both of the methods for learning constraints are complex and time-demanding. 


Regarding the generation of the constrained examples, in the first study \cite{sheatsley2020adversarial} selects the most salient feature to perturb and applies constraint resolution. Once the feature for perturbation is selected based on saliency value, a check is made to see if it is realted to any primary features and a set of violated constraints if any is located. So the constraints are enforced at crafting step.
In the second study \cite{sheatsley2021robustness} they introduced Constrained-Saliency Projection  an iterative attack who selects the most influential feature to perturb based in saliency maps calculated by AJSMA. The updated sample is projected back to the constraint space learned by Valiant's algorithm through an existing algorithm for constraint satisfaction named Davis-Putnam-Logeman-Loveland (DPLL). 



\cite{levy2020not} updates JSMA attack to take into account immutable features and feature distribution. At each iteration the most influential feature on the model prediction is selected. The perturbation added to this features is found through ADAM optimizer. Finally  each feature of the new sample is  updated such it respects its probability distribution. This approach despite claiming that deals with validity of adversarial examples in constrained domains, handles very loose constraints like mutability and probability distributions. It does not specifically consider inter-feature relationships and the constraints that come with that.  



\textbf{Extended Carlini and Wagner (C&W) attack}
Carlini & Wagner \cite{carlini2017towards} expressed the problem of generating adversarial examples as an optimization problem where the objective function tries to maximize the 
target prediction, while minimising the size of the perturbation. In the minimisation term \cite{teuffenbach2020subverting} introduced weights for features based on the difficulty to attack them while preserving the constraints. Features with same difficulty are grouped together and assigned the same weight. The higher the weights the higher the difficulty that an adversary faces to change them and preserve constraints. For example a weight of 1 is given to features that are independent and whose value does not influence other features. A weight of 3 is given to features that involve physical constraints for an attacker such as time. The extended C&W proposed by \cite{teuffenbach2020subverting} favours the modifications of low weight features in this case independent features. However the drawback  if the algorithm can not generate an adversarial by modifying low weight features and tries to add small modification to higher weight features, this approach has no guarantee that the modifications will respect the intra-features relationships. It relies heavily on in the hopes that the modifications of low weight features will be enough to generate adversarials. Addittionally a domain expert is needed to decide groups of features and their weights. 



\textbf{Constraint-based IFGSM (C-IFGSM)}

\cite{tian2020exploring} explores visually feature correlations between features pairs. If any correlation is observed, then the constraint equation is defined analytically. The visualization handles four type of constraints: strict linear constraints, zero multiplication constraints, addittion boundary constraints, approximate linear constraints.  For every step of IFGSM a constraint matrix is generated dynamically according to the constraint set and the sign of the gradient.  The Hadambard product between the sign of the gradient and constraint matrix  restricts the size  and direction of perturbation to respect data correlations. Despite this  method being among the few that uses a large variety of constraints types, it can not handle relationships of more than two features. Addittionally, visual explorations of feature correlations is not scalable when the number of features increases in the large datasets. The advantage of this approach however is that it would be relatively easily to adapt it to the new doamins. A domain expert is not necessary, but a person with basic knowledge in correlations is needed to analyze visually the feature relationships and define the constraint equations. The rest of the steps on how to create the constraint matrix are reusable and clearly defined in the original paper despite the fact that the code of C-IGSM is not open source. 

\textbf{Graphical Framework}

For constrained discrete domains, \cite{kulynych2018evading} proposes a graphical framework to search for valid adversarial examples.  A transformation graph is defined before execution
where the nodes represent the feasible examples and the edges represent valid transformations of one feature that connect an original sample $x$ and its perturbed version $x'$. Each tranformation has a cost that is expressed as a weight for the edge. They use A* graph search algorithm to find an adversarial example with minimum transformation costs. This approach is one of most innovative approaches proposed for generation of constrained domains. However, it has some drawbacks. Firstly, in order to build the transformation graphs it needs to preprocess the features such all of them are one-hot-encoded. So the approach works best for datasets with discrete features. For continuous features the authors propose to split them in range of values (buckets). However, this might lead to non-realistic samples. Secondly, a domain expert is needed to define the weights for every transformation. Thirdly, the graph size increases with the number of features, so increases the run time for A*. This makes this approach not scalable to large datasets.



 
\textbf{ConAML}

\cite{li2020conaml} designed a best effort search algorithm to iteratively generate adversarial examples
that respect linear physical constraints derived from Cyber-Physical Systems application domain.  ConAML supports  linear equality and non-equality constraints  in addition to simple constraints like mutability and range. The general best effort search algorithm for linear equalities starts by initializing the perturbation vector. Until a maximum number of iterations, the perturbation vector is increased by a perturbation r that matches the constraints. r is calculated as follows. From the constraints' matrix we identify the independent variables, dependent variables and a dependency matrix between them. We use the gradient values of independent variables and use them to compute the values of dependent variables. The final perturbation respect so the linear constraints. A modified version of this algorithm is given in this paper for non-linear constraints as well. 

The threat model of this attack is closely related to CPS. Hence, adapting to other use cases in CPS would be feasible. Meanwhile, adapting it to other domains would require to define the threat model and update the algorithm accordingly. One drawback of the approach is that it can not deal with non-linear constraints. 





\subsection{Black-box}

\textbf{Genetic Algortihm: Coeva2}

The proposed constrained black-box attacks are less numerous. First, \cite{ghamizi2020search} proposes a black box attack based on the genetic algorithm that encodes constraints as objectives to be optimized.
Coeva2 creates a population of individuals based on an initial state. The population has same values for the immutable features, they differ only on mutable ones. The generated samples in the population  respect  the feature range constraints and data type constraints. This population evolves for a predefined number of generations through selection, crossover and mutation operators trying to optimize the values for the fitness functions. Their four objectives are expressed as a function. 1) Maximize the probability that the example is classified as target class 2) Minimize the perturbation 3) Maximize some business objective 4)Satisfy domain constraints. During the evolution process they allow the generation of samples that do not respect constraints in order to explore  a larger search space. However the fourth objective makes sure that during the evolution process the samples that respects the constraints are more preferred. 

This approach supports a variety of linear, non-linear and statistical constraints as long as they can be expressed as a minimization problem. However, being that this is a multi-objective search a domain expert is needed to define the weights given to each objective or tuning of the weights is required. 


\textbf{Modified: Zoo, Boundary attack, HopSkipJump}
\cite{cartella2021adversarial} investigated three existing black-box adversarial attacks (Zoo, Boundary attack, HopSkipJump)[insert citations here] and observed that they are not ready for tabular and imbalanced data. They proposed a few modifications that will make these attacks generate more constrained adversarial examples.
For imbalanced data like the case of fraud detection, the classification threshold is originally fine-tuned to count for class imbalance. Originally Zoo, Boundary attack, HopSkipJump were using a threshold of 0.5, which makes it believe that adversarial examples were found when that was not the case. \cite{cartella2021adversarial} modified these algorithms to include custom thresholds. The next modification included a custom loss function for Zoo attack. Similarly to the above threshold problem, Zoo uses a loss function that assumes a standard threshold of 0.5. The newly introduced loss function ensures that the minimum values of loss are reached only when the classification of the adversarial examples is below the threshold. They modified the algorithms to respect data type constraints. Finally, the last modification is related to define a custom edit norm that is not the traditional Lp norms used for the images. The new norm gives weight to the features based on two main factors a) if the feature is checked by a human operator b) the importance of the feature for the model. 


The modifications made by \cite{cartella2021adversarial} restrict the space of generated adversarial examples, but unfortunately do not take in consideration if some relationships exist between features. Therefore, the resulting examples are still probable to not be feasible or valid. However, the point they raise on custom norms is interesting and valuable. Many studies in constrained domains import the Lp norms from the image domain, when sometimes the threat model does not support this norm. 


In addition to these two works, \cite{kulynych2018evading, li2020conaml} presented in their papers adapted approaches of their works for black-box scenarios. 


The field of constrained adversarial attacks in feature space is relatively new. The first attack that explicitly mention feature constraints was proposed by \cite{chernikova2019fence} in 2018. Despite that each year, new constrained attacks emerge, many of them handles only basic constraints like mutability or data type. These types of constraints restrict the generated adversarial examples, but do not completely ensure that they are feasible and realistic. There is a need for constrained attacks that are suitable for many domains and at the same time support a large variety of constraints. You can find a complete list of constrained adversarial attacks and their properties in Table \ref{tab-cons-attacks}

\begin{table*}[ht!]
\centering
\caption{Adversarial attacks in feature space that consider domain constraints}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllll} 
\toprule
                                                  & Year & Use case                         & Threat model     & Method                                & Constraint type                 & Expansion to new domains    & Open source  \\ 
\midrule
\cite{kulynych2018evading}    & 2018 & Twitter bot                      & White  Black box & Graphical framework                   & Mutability                      & Define~                     & Yes          \\
                                                  &      & Website-fingerprinting           &                  &                                       & Modification step               & the transformation graph    &              \\ 
\hline
\cite{chernikova2019fence}       & 2019 & Botnet detection                 & White box        & Iterative Gradient Based               & Mutability, Range,              & Rewrite most~               & Yes          \\
                                                  &      & Malicious domain classification  &                  &                                       & Ratio,One-hot encoding          & of the components           &              \\
                                                  &      &                                  &                  &                                       & Statistical ,Linear, Non-linear &                             &              \\ 
\hline
\cite{ghamizi2020search}         & 2020 & Credit scoring                   & Grey-box         & Genetic Algorithm                     & Mutability, Range,              & Define constraints~         & Yes          \\
                                                  &      &                                  &                  &                                       & Ratio, One-hot-encoding,        & as a minimization problem   &              \\
                                                  &      &                                  &                  &                                       & statistical, linear, non-linear &                             &              \\ 
\hline
\cite{li2020conaml}              & 2020 & Water treatment attack detection & White black box  & Best-Effort Search                    & Mutability,range                & Define constraints          & No           \\
                                                  &      & State Estimation in Power Grids  &                  &                                       & Linear, 
Simple non-linear      &                             &              \\ 
\hline
\cite{levy2020not}               & 2020 & price of lodging (AirBnb)        & White-box        & Extended JSMA                         & Mutability, Range,              & Yes                         & No           \\
                                                  &      & medical data ICU                 &                  &                                       &                                 &                             &              \\
                                                  &      & credit risk                      &                  &                                       &                                 &                             &              \\ 
\hline
\cite{sheatsley2020adversarial}  & 2020 & NIDS                             & White-box        & Constrained Augmented JSMA            & Mutability,Range,               & Learn constraints~          & No           \\
                                                  &      &                                  &                  &                                       & Boolean                         & from data                   &              \\ 
\hline
\cite{teuffenbach2020subverting} & 2020 & NIDS                             & White-box        & Extended CW attack                    & Mutability                      & Define feature groups       & No           \\ 
\hline
\cite{tian2020exploring}         & 2020 & NIDS                             & White-box        & Constraint-based IFGSM                & Linear                          & Define constraints~         & No           \\
                                                  &      &                                  &                  &                                       & Addition boundary constraint,   & by visual exploration       &              \\
                                                  &      &                                  &                  &                                       & Zero multiplication constraint  &                             &              \\ 
\hline
\cite{cartella2021adversarial}   & 2021 & Fraud                            & Black box        & 3 modified black-box attacks          & Mutability,Data type            & Define feature weights      & No           \\ 
\hline
\cite{sheatsley2021robustness}   & 2021 & NIDS,                            & White-box        & Constrained Saliency Projection & Boolean constraints             & Learn constraints~          & No           \\
                                                  &      & Phishing                         &                  &                                       &                                 & through Valiant’s algorithm &              \\
\bottomrule
\end{tabular}}
\label{tab-cons-attacks}
\end{table*}


\subsection{Limitations and future work}



